USDRL: Unified Skeleton-Based Dense Representation Learning with Multi-Grained Feature Decorrelation

Contrastive learning has achieved great success in skeleton-based representation learning recently. However, the prevailing methods are predominantly negative-based, necessitating additional momentum encoder and memory bank to get negative samples, which increases the difficulty of model training. Furthermore, these methods primarily concentrate on learning a global representation for recognition and retrieval tasks, while overlooking the rich and detailed local representations that are crucial for dense prediction tasks. To alleviate these issues, we introduce a Unified Skeleton-based Dense Representation Learning framework based on feature decorrelation, called USDRL, which employs feature decorrelation across temporal, spatial, and instance domains in a multi-grained manner to reduce redundancy among dimensions of the representations to maximize information extraction from features. Additionally, we design a Dense Spatio-Temporal Encoder (DSTE) to capture fine-grained action representations effectively, thereby enhancing the performance of dense prediction tasks. Comprehensive experiments, conducted on the benchmarks NTU-60, NTU-120, PKU-MMD I, and PKU-MMD II, across diverse downstream tasks including action recognition, action retrieval, and action detection, conclusively demonstrate that our approach significantly outperforms the current state-of-the-art (SOTA) approaches. Our code and models are available at https://github.com/wengwanjiang/USDRL.

==> checklist.tex <==

\section{Reproducibility Checklist}
Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.
\begin{enumerate}
\item This paper
\begin{enumerate}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) yes
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) yes
  \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) yes

\end{enumerate}
\item Does this paper make theoretical contributions? (yes/no) no

If yes, please complete the list below.
\begin{enumerate}
  \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
  \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
  \item Proofs of all novel claims are included. (yes/partial/no)
 \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
 \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
 \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
 \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{enumerate}
\item Does this paper rely on one or more datasets? (yes/no) yes

If yes, please complete the list below.
\begin{enumerate}
 \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) yes
 \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) NA
 \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) NA
 \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) yes
 \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) yes
 \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) NA
\end{enumerate}
\item Does this paper include computational experiments? (yes/no) yes

If yes, please complete the list below.
\begin{enumerate}
 \item Any code required for pre-processing data is included in the appendix. (yes/partial/no). no
 \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) no
 \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) yes
 \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) yes
 \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) yes
 \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) no
 \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) no
 \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) no
 \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) no
 \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) no
 \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) yes
 \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) no
\end{enumerate}
\end{enumerate}


==> table/abl_encoder_layer.tex <==
% Table generated by Excel2LaTeX from sheet 'linear'
\begin{table}[htbp]
  \centering
    \begin{tabular}{ccccc}
    \toprule
    Layer Num & Para. (M) & Recognition & Retrieval \\
    \midrule
    1     & 67.7 & 84.5     & 73.1 \\
    2     & 94.9 & 85.2  & 75.0 \\
    3     & 113.9 & 84.9      & 75.4 \\
    \bottomrule
    \end{tabular}
      \caption{The study on the impact of the number of encoder layers. The performance is evaluated on the NTU60 X-sub dataset under the linear evaluation protocol.}
  \label{tab:abl_encoder_layer}
\end{table}


==> table/ntu2pku.tex <==
% Table generated by Excel2LaTeX from sheet 'linear'
\begin{table}[htbp]
  \centering
    \begin{tabular}{lcc}
    \toprule
    \multirow{2}[4]{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Transfer to PKU-MMD II}} \\
\cmidrule{2-3}          & \textbf{NTU-60} & \textbf{NTU-120} \\
    \midrule
    % LongT GAN~\shortcite{zheng2018unsupervised} & 44.8  & - \\
    MS$^\text{2}$L~\shortcite{MS2L}  & 45.8  & - \\
    ISC~\shortcite{thoker2021skeleton}   & 45.9  & - \\
    SCD-Net~\shortcite{wu2024scd} & 56.3  & - \\
    HiCo~\shortcite{hico2023}  & 56.3  & 55.4 \\
    CMD~\shortcite{mao2022cmd}    & 56    & 57 \\
    UmURL~\shortcite{sun2023unified} & 58.2  & 57.6 \\
    \midrule
    \textbf{USDRL} & \textbf{57.2} & \textbf{58.3} \\
    \bottomrule
    \end{tabular}
      \caption{Comparisons of transfer learning results when transferring to PKU-MMD II.}
  \label{ntu2pku}
\end{table}

